Auxiliary-task learning for geographic data with autoregressive embeddings

Machine learning is gaining popularity in a broad range of areas working with geographic data, such as ecology or atmospheric sciences. Here, data often exhibit spatial effects, which can be difficult to learn for neural networks. In this study, we propose SXL, a method for embedding information on the autoregressive nature of spatial data directly into the learning process using auxiliary tasks. We utilize the local Moran's I, a popular measure of local spatial autocorrelation, to "nudge" the model to learn the direction and magnitude of local spatial effects, complementing the learning of the primary task. We further introduce a novel expansion of Moran's I to multiple resolutions, thus capturing spatial interactions over longer and shorter distances simultaneously. The novel multi-resolution Moran's I can be constructed easily and as a multi-dimensional tensor offers seamless integration into existing machine learning frameworks. Throughout a range of experiments using real-world data, we highlight how our method consistently improves the training of neural networks in unsupervised and supervised learning tasks. In generative spatial modeling experiments, we propose a novel loss for auxiliary task GANs utilizing task uncertainty weights. Our proposed method outperforms domain-specific spatial interpolation benchmarks, highlighting its potential for downstream applications. This study bridges expertise from geographic information science and machine learning, showing how this integration of disciplines can help to address domain-specific challenges. The code for our experiments is available on Github: https://github.com/konstantinklemmer/sxl.

==> impact.tex <==
\section*{Broader Impact}

As our paper is motivated by real-world problems, it is naturally close to applications and may have a real impact on practitioners in the geospatial domain. Where these industry or public sector applications overlap with social systems, our study might impact society on a broader scale. 

\textit{Positive Impact:} Our main motivation for this research are urgent calls-to-action \citep{Reichstein2019,Janowicz2020}, calling for better deep learning tools for geospatial domains. Deep learning in particular offers a novel pathway for modeling our geophysical environment more pervasively than ever before---helping us respond to existential threats such as climate change. Stepping back from the ``big picture'', there are also smaller, but potentially life-saving applications which might benefit from our research, such as modeling crop yields or forecasting earthquake and hurricane trajectories. Lastly, we also hope that further connecting the machine learning community with other sciences (in our case geography) will help with creating machine learning solutions for real-world problems, accounting for the vast prior knowledge on social complexities provided by the social sciences. 

\textit{Risks:} As we provide a general tool for geospatial modeling, we can also imagine harmful application scenarios. In particular, \texttt{SXL} could be utilized in geospatial analytics tasks related to the defense industry. Satellite and UAV reconnaissance systems often rely on analytics tools and other software to process raw data---including, for example, spatial interpolation capabilities. Beyond military applications, and since we earlier highlighted how we believe our study can help tackle the climate crisis, it is important to mention here that another industry heavily relying on geospatial intelligence is the fossil fuel industry, where geospatial analytics are used for e.g. coal mining and fracking. 
